Med-StepBench: A Hierarchical Reasoning Framework for Evaluating Hallucinations in Medical Vision-Language Models

Large vision-language models (VLMs) demonstrate strong performance in medical image understanding, but frequently generate clinically plausible yet incorrect statements, raising significant safety concerns. Existing medical hallucination benchmarks primarily focus on 2D imaging with one-shot diagnostic questions, offering limited insight into whether predictions are grounded in correct localization and abnormality identification, allowing critical reasoning errors to remain hidden behind seemingly correct diagnoses. We introduce Med-StepBench, the first large-scale benchmark for step-wise hallucination detection in 3D oncological PET/CT, comprising over 12,000 images and more than 1,000,000 image-statement pairs across volumetric and multi-view 2D data, which decomposes clinical reasoning into four expert-designed diagnostic stages. Using clinician-verified annotations, we perform the first step-level evaluation of general-purpose and medical VLMs, revealing systematic failure modes obscured by aggregate accuracy metrics. Furthermore, we show that current VLMs are highly susceptible to adversarial yet clinically plausible intermediate explanations, which significantly amplify hallucinations despite contradictory visual evidence. Together, our findings highlight fundamental limitations in grounding multi-step clinical reasoning and establish Med-StepBench as a rigorous benchmark for developing safer and more reliable medical VLMs.

==> Document/5.1.tex <==



% We also observe that knowledge injection for both types of knowledge only yields marginal F1 changes for most models in most steps, and does not help to alleviate hallucination meaningfully. Step 2 generally yields small F1 gains or remains unchanged, indicating that contextual constraints align well with lesion presence verification, though occasional degradations (e.g., LLaVA-Med) suggest limited robustness. In contrast, Step 3 shows little improvement and frequent drops, highlighting a persistent bottleneck where lightweight prompts fail to support fine-grained attribute grounding and models revert to textual priors. Step 4 typically improves or stays flat, but gains are largely driven by a precision–recall trade-off, with higher sensitivity accompanied by increased false positives. Overall, intermediate knowledge primarily redistributes errors rather than achieving consistent hallucination reduction, benefiting lesion identification more than feature characterization.
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/EN_VI_doublebar_dumbbell2.png}
%     \caption{Performance of models between Vietnamese \& English dataset}
%     \label{fig:placeholder}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/Models_steps_comparision2.png}
%     \caption{Performance of models during steps (F1-score).}
% %    \Amir{It is better you give me the table information with 2 floating points, so on top of the bar, I update the percentage with 2 floating points}
%     \label{fig:step_wise}
% \end{figure}


% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.2pt}
% \renewcommand{\arraystretch}{1.15}

% \begin{tabular}{lccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} 
% & \multicolumn{3}{c|}{\textbf{Special}} 
% & \multicolumn{3}{c|}{\textbf{Easy}} 
% & \multicolumn{3}{c}{\textbf{Hard}} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
% & P & R & F1 & P & R & F1 & P & R & F1 \\
% \midrule

% Med-Flamingo
% & 0.43 & 0.76 & 0.55
% & 0.49 & 0.84 & 0.62
% & 0.20 & 0.24 & 0.22 \\

% Gemini Pro
% & 0.48 & 0.70 & 0.57
% & 0.50 & 0.88 & 0.64
% & 0.51 & 0.96 & 0.67 \\

% Gemini Flash
% & 0.47 & 0.74 & 0.57
% & 0.50 & 0.96 & 0.66
% & 0.53 & 0.98 & 0.69 \\

% % GPT-4o
% % & 0.48 & 0.84 & 0.61
% % & --   & --   & --
% % & --   & --   & -- \\

% MedM 3D
% & 0.42 & 0.72 & 0.53
% & 0.48 & 0.90 & 0.63
% & 0.47 & 0.86 & 0.60 \\

% MedM 2D
% & 0.37 & 0.58 & 0.45
% & 0.38 & 0.60 & 0.46
% & 0.36 & 0.57 & 0.45 \\

% \bottomrule
% \end{tabular}

% \caption{Hallucination detection performance under different test settings}
% \label{tab:hallu_results_split}

% \end{table}



% - main hallucination when model fail at detecting FDG uptake physically or abnormaility

==> Document/5.2.tex <==
% In this experiment, we provide the VLMs with two types of knowledges: \textit{Prior Knowledge} from previous steps and \textit{External Knowledge}
% \textit{Prior knowledge} obtained by previous steps of the diagnostic process helps improve the Hallucination Detection performance. For example, when conducting the Hallucination Detection for Step 4, Diagnostic Synthesis, we also feed VLMs the ground truth description of Step 3, Feature Characterization. \\
% We observe that knowledge injection for both types of knowledge only yields marginal F1 changes for most models in most steps, and does not help to alleviate hallucination meaningfully. Step 2 generally yields small F1 gains or remains unchanged, indicating that contextual constraints align well with lesion presence verification, though occasional degradations (e.g., LLaVA-Med) suggest limited robustness. In contrast, Step 3 shows little improvement and frequent drops, highlighting a persistent bottleneck where lightweight prompts fail to support fine-grained attribute grounding and models revert to textual priors. Step 4 typically improves or stays flat, but gains are largely driven by a precision–recall trade-off, with higher sensitivity accompanied by increased false positives. Overall, intermediate knowledge primarily redistributes errors rather than achieving consistent hallucination reduction, benefiting lesion identification more than feature characterization.
% The effect is step-dependent: Step 2 typically improves slightly, Step 3 often fails to improve (and can drop), while Step 4 shows clearer gains that are largely driven by a precision–recall trade-off.

% In Step 2 (Lesion Identification), most models either increase F1 slightly or remain unchanged, suggesting that simple contextual cues and constraints are relatively well-aligned with presence/absence verification. However, this benefit is not guaranteed, as some models can still degrade (e.g., LLaVA-Med), indicating that knowledge injection is not universally helpful.

% In Step 3 (Feature Characterization), many models do not improve and some deteriorate, implying that adding lightweight intermediate prompts is insufficient for the fine-grained grounding required by attribute-level or quantitative characterization.This stage remains the most persistent bottleneck because models can fall back on textual priors rather than extracting deeper evidence from the image.

% In Step 4 (Diagnostic Synthesis), most models improve or stay flat, but the gains commonly coincide with lower precision and higher recall, meaning models become more sensitive to inconsistencies while also producing more false alarms.

% Overall, intermediate knowledge primarily shifts the error profile rather than delivering consistent, step-wide reductions in hallucination, and its utility is more apparent for Step 2 than for the attribute-grounding demands of Step 3.

% Requires: \usepackage{booktabs,adjustbox,multirow}




==> Document/5.3.tex <==
\subsection{Effects of Prior and External Knowledge}
\paragraph{\hyperref[rq:knowledge]{RQ3}.}
% \reza{to refer the labels of RQs, pls use \hyperref[rq:knowledge]{RQ3}, I am fixing this but pls check all places to reffer the RQs}
% Requires: \usepackage{booktabs,adjustbox,multirow}
% \begin{table}[h]
% \centering
% \label{tab:internal_vs_external}
% \tiny
% \setlength{\tabcolsep}{1.4pt}
% \renewcommand{\arraystretch}{1.12}
% \begin{adjustbox}{width=1\columnwidth}
% \begin{tabular}{l !{\vrule width 0.8pt} l !{\vrule width 0.8pt}
% ccc !{\vrule width 0.8pt}
% ccc !{\vrule width 0.8pt}
% ccc}
% \hline
% \textbf{Model} & \textbf{Src} &
% \multicolumn{3}{c!{\vrule width 0.8pt}}{\textbf{Step 2}} &
% \multicolumn{3}{c!{\vrule width 0.8pt}}{\textbf{Step 3}} &
% \multicolumn{3}{c}{\textbf{Step 4}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% & & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline

% \multirow{4}{*}{Qwen3-VL-4B}
% & None 
% & 0.58 & 0.82 & 0.68 
% & 0.51 & \textbf{0.94} & 0.66 
% & 0.62 & 0.65 & 0.63 \\
% & +Prior      
% & 0.53 & \textbf{0.94} & 0.68 
% & 0.58 & 0.72 & 0.64 
% & \textbf{0.63} & 0.83 & \textbf{0.72} \\
% & +Ext      
% & \textbf{0.60} & 0.88 & \textbf{0.71} 
% & 0.54 & 0.78 & 0.64 
% & 0.55 & 0.50 & 0.52 \\
% & +Both    
% & 0.59 & 0.84 & 0.69 
% & \textbf{0.59} & 0.78 & \textbf{0.67} 
% & 0.55 & \textbf{0.88} & 0.67 \\
% \hline

% \multirow{4}{*}{Med-Flamingo}
% & None 
% & 0.63 & 0.69 & 0.66 
% & \textbf{0.51} & 0.82 & 0.63 
% & 0.53 & 0.67 & 0.59 \\
% & +Prior      
% & 0.55 & 0.94 & \textbf{0.70} 
% & 0.50 & \textbf{0.88} & \textbf{0.64} 
% & 0.54 & \textbf{0.79} & \textbf{0.64} \\
% & +Ext      
% & 0.55 & \textbf{0.96} & \textbf{0.70} 
% & 0.47 & 0.80 & 0.59 
% & 0.52 & 0.77 & 0.62 \\
% & +Both    
% & \textbf{0.65} & 0.74 & 0.69 
% & 0.47 & 0.82 & 0.59 
% & \textbf{0.55} & 0.71 & 0.62 \\
% \hline

% \multirow{4}{*}{Gemini 2.5 flash}
% & None 
% & 0.65 & 0.82 & \textbf{0.72} 
% & 0.56 & \textbf{0.84} & \textbf{0.67} 
% & \textbf{0.64} & 0.58 & 0.61 \\
% & +Prior      
% & 0.52 & 0.65 & 0.58 
% & 0.50 & 0.58 & 0.54 
% & 0.62 & 0.63 & 0.63 \\
% & +Ext      
% & 0.63 & \textbf{0.85} & \textbf{0.72} 
% & 0.57 & 0.82 & \textbf{0.67} 
% & 0.60 & 0.72 & \textbf{0.65} \\
% & +Both    
% & \textbf{0.66} & 0.80 & \textbf{0.72} 
% & \textbf{0.58} & 0.78 & \textbf{0.67} 
% & 0.57 & \textbf{0.77} & \textbf{0.65} \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Different knowledge input across steps. \textbf{+Prior}: prior knowledge, \textbf{+Ext}: external knowledge.}
% \end{table}

% \begin{table}[h]
% \centering
% \label{tab:internal_vs_external}
% \tiny
% \setlength{\tabcolsep}{1.7pt}
% \renewcommand{\arraystretch}{1.12}

% \begin{adjustbox}{width=1\columnwidth}
% \begin{tabular}{l !{\vrule width 0.8pt} l !{\vrule width 0.8pt}
% ccc !{\vrule width 0.8pt}
% ccc !{\vrule width 0.8pt}
% ccc}
% \hline
% \textbf{Model} & \textbf{Src} &
% \multicolumn{3}{c!{\vrule width 0.8pt}}{\textbf{Step 2}} &
% \multicolumn{3}{c!{\vrule width 0.8pt}}{\textbf{Step 3}} &
% \multicolumn{3}{c}{\textbf{Step 4}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% & & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline

% \multirow{4}{*}{\makecell[c]{Qwen3\\VL-4B}}
% & None 
% & 0.58 & 0.82 & 0.68 
% & 0.51 & \textbf{0.94} & 0.66 
% & 0.62 & 0.65 & 0.63 \\
% & +Prior      
% & 0.53 & \textbf{0.94} & 0.68 
% & 0.58 & 0.72 & 0.64 
% & \textbf{0.63} & 0.83 & \textbf{0.72} \\
% & +Ext      
% & \textbf{0.60} & 0.88 & \textbf{0.71} 
% & 0.54 & 0.78 & 0.64 
% & 0.55 & 0.50 & 0.52 \\
% & +Both    
% & 0.59 & 0.84 & 0.69 
% & \textbf{0.59} & 0.78 & \textbf{0.67} 
% & 0.55 & \textbf{0.88} & 0.67 \\
% \hline

% \multirow{4}{*}{\makecell[c]{Med\\Flamingo}}
% & None 
% & 0.63 & 0.69 & 0.66 
% & \textbf{0.51} & 0.82 & 0.63 
% & 0.53 & 0.67 & 0.59 \\
% & +Prior      
% & 0.55 & 0.94 & \textbf{0.70} 
% & 0.50 & \textbf{0.88} & \textbf{0.64} 
% & 0.54 & \textbf{0.79} & \textbf{0.64} \\
% & +Ext      
% & 0.55 & \textbf{0.96} & \textbf{0.70} 
% & 0.47 & 0.80 & 0.59 
% & 0.52 & 0.77 & 0.62 \\
% & +Both    
% & \textbf{0.65} & 0.74 & 0.69 
% & 0.47 & 0.82 & 0.59 
% & \textbf{0.55} & 0.71 & 0.62 \\
% \hline

% \multirow{4}{*}{\makecell[c]{Gemini \\2.5\\Flash}}
% & None 
% & 0.65 & 0.82 & \textbf{0.72} 
% & 0.56 & \textbf{0.84} & \textbf{0.67} 
% & \textbf{0.64} & 0.58 & 0.61 \\
% & +Prior      
% & 0.52 & 0.65 & 0.58 
% & 0.50 & 0.58 & 0.54 
% & 0.62 & 0.63 & 0.63 \\
% & +Ext      
% & 0.63 & \textbf{0.85} & \textbf{0.72} 
% & 0.57 & 0.82 & \textbf{0.67} 
% & 0.60 & 0.72 & \textbf{0.65} \\
% & +Both    
% & \textbf{0.66} & 0.80 & \textbf{0.72} 
% & \textbf{0.58} & 0.78 & \textbf{0.67} 
% & 0.57 & \textbf{0.77} & \textbf{0.65} \\
% \hline
% \end{tabular}
% \end{adjustbox}

% \caption{Different knowledge input across steps. \textbf{+Prior}: prior knowledge, \textbf{+Ext}: external knowledge.}
% \end{table}
We also observe that knowledge injection for both types of knowledge only yields marginal F1 changes for most models in most steps, and does not help to alleviate hallucination meaningfully (Table~\ref{tab:internal_vs_external}) . Step 2 generally yields small F1 gains or remains unchanged, indicating that contextual constraints align well with lesion presence verification, though occasional degradations (e.g., LLaVA-Med) suggest limited robustness. In contrast, Step 3 shows little improvement and frequent drops, highlighting a persistent bottleneck where lightweight prompts fail to support fine-grained attribute grounding and models revert to textual priors. Step 4 typically improves or stays flat, but gains are largely driven by a precision–recall trade-off, with higher sensitivity accompanied by increased false positives. Overall, intermediate knowledge primarily redistributes errors rather than achieving consistent hallucination reduction, benefiting lesion identification more than feature characterization.


\begin{table}[h]
\centering

\tiny
\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.22}

\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{l| cc| ccc |ccc| ccc}
\hline
\textbf{Model} &
\multicolumn{2}{c|}{\textbf{Knowledge}} &
\multicolumn{3}{c|}{\textbf{Step 2}} &
\multicolumn{3}{c|}{\textbf{Step 3}} &
\multicolumn{3}{c}{\textbf{Step 4}} \\
%\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
\hline
& \textbf{Prior} & \textbf{Ext} &
\textbf{P} & \textbf{R} & \textbf{F1} &
\textbf{P} & \textbf{R} & \textbf{F1} &
\textbf{P} & \textbf{R} & \textbf{F1} \\
\hline
\multirow{4}{*}{\makecell[c]{Qwen3\\VL-4B}}
&  & 
& 0.58 & 0.74 & 0.65
& 0.56 & 0.70 & 0.62
& 0.62 & 0.65 & 0.63 \\
& \cmark & 
& 0.53 & \textbf{0.94} & 0.68
& 0.58 & 0.72 & 0.64
& \textbf{0.63} & 0.83 & \textbf{0.72} \\
&  & \cmark
& \textbf{0.60} & 0.88 & \textbf{0.71}
& 0.54 & 0.78 & 0.64
& 0.55 & 0.50 & 0.52 \\
& \cmark & \cmark
& 0.59 & 0.84 & 0.69
& \textbf{0.59} & 0.78 & \textbf{0.67}
& 0.55 & \textbf{0.88} & 0.67 \\
%\addlinespace[2.5pt]
\hline
%\addlinespace[1pt]
\multirow{4}{*}{\makecell[c]{Med\\Flamingo}}
&  &
& 0.63 & 0.69 & 0.66
& \textbf{0.51} & 0.82 & 0.63
& 0.53 & 0.67 & 0.59 \\
& \cmark &
& 0.55 & 0.94 & 0.70
& 0.50 & \textbf{0.88} & \textbf{0.64}
& 0.54 & \textbf{0.79} & \textbf{0.64} \\
&  & \cmark
& 0.55 & \textbf{0.96} & \textbf{0.70}
& 0.47 & 0.80 & 0.59
& 0.52 & 0.77 & 0.62 \\
& \cmark & \cmark
& \textbf{0.65} & 0.74 & 0.69
& 0.47 & 0.82 & 0.59
& \textbf{0.55} & 0.71 & 0.62 \\
%\addlinespace[2.5pt]
\hline
%\addlinespace[1pt]
\multirow{4}{*}{\makecell[c]{Gemini\\ 2.5\\Flash}}
&  &
& 0.65 & 0.82 & \textbf{0.72}
& 0.56 & \textbf{0.84} & \textbf{0.67}
& \textbf{0.64} & 0.58 & 0.61 \\
& \cmark &
& 0.52 & 0.65 & 0.58
& 0.50 & 0.58 & 0.54
& 0.62 & 0.63 & 0.63 \\
&  & \cmark
& 0.63 & \textbf{0.85} & \textbf{0.72}
& 0.57 & 0.82 & \textbf{0.67}
& 0.60 & 0.72 & \textbf{0.65} \\
& \cmark & \cmark
& \textbf{0.66} & 0.80 & \textbf{0.72}
& \textbf{0.58} & 0.78 & \textbf{0.67}
& 0.57 & \textbf{0.77} & \textbf{0.65} \\

\hline
\end{tabular}
\end{adjustbox}

\caption{Different knowledge input across steps. Prior/Ext indicate whether prior knowledge or external knowledge is provided (both checked means +Both; none checked means no knowledge).}
\label{tab:internal_vs_external}
\end{table}



% The goal of this experiment is to examine the effects of prior knowledge  from previous steps and external knowledge on hallucination detection in Steps 2–4. We compare four settings—without / internal / external / both—on the same set of samples and report precision, recall, and F1 for each step. Overall, the impact of knowledge is model-dependent, and no single choice is consistently optimal. For general VLMs (e.g., Qwen3-VL-4B, Gemini 2.5 Flash), external knowledge is often more beneficial because it provides clinical criteria and medical context that general-purpose models do not reliably capture. In contrast, for Med-Flamingo, internal (sequential) knowledge tends to be more suitable, as it helps maintain step-wise reasoning coherence and reduces drift in later stages. The both setting is not always superior because internal and external signals can introduce noise or conflict, leading to unstable gains. External knowledge often makes models more “sensitive” by increasing recall, but it can sometimes reduce precision, so F1 may not improve proportionally. By step, external knowledge typically aligns better with Step 2, where clinical criteria are needed to verify lesion presence or absence, whereas internal knowledge is often more important for Steps 3–4, which require consistent reasoning grounded in the validated context from the previous step. In summary, general models benefit more from external medical knowledge to mitigate domain gaps, while medical models benefit more from internal sequential constraints to improve step-wise consistency.


%\subsubsection{RQ\ref{rq:fusion}: Clinically Aligned PET/CT Fusion}
\subsection{Clinically Aligned PET/CT Fusion}
\paragraph{\hyperref[rq:fusion]{RQ4}}

%\hyperref[rq:fusion]{RQ4}

% \begin{table}[H]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3.2pt}
% \renewcommand{\arraystretch}{1.15}

% \begin{adjustbox}{width=\columnwidth}
% \begin{tabular}{l !{\vrule width 0.8pt} c !{\vrule width 0.8pt}
% cc !{\vrule width 0.8pt}
% cc !{\vrule width 0.8pt}
% cc !{\vrule width 0.8pt}
% cc}
% \hline
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Input}} &
% \multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 1}} &
% \multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 2}} &
% \multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 3}} &
% \multicolumn{2}{c}{\textbf{Step 4}} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
% & & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} \\
% \hline

% \multirow{2}{*}{Med-Flamingo}
% & PET + CT
% & -- & 0.64 & -- & 0.64 & -- & \textbf{0.66} & -- & \textbf{0.66} \\
% & PET/CT
% & -- & \textbf{0.77}\textcolor[HTML]{008000}{$\uparrow$} 
% & -- & \textbf{0.66}\textcolor[HTML]{008000}{$\uparrow$} 
% & -- & 0.63\textcolor[HTML]{FF0000}{$\downarrow$} 
% & -- & 0.59\textcolor[HTML]{FF0000}{$\downarrow$} \\
% \hline

% \multirow{2}{*}{Gemini 2.5 Flash}
% & PET + CT
% & 0.79 & 0.81 & 0.68 & \textbf{0.72} & 0.62 & 0.62 & 0.51 & 0.52 \\
% & PET/CT
% & \textbf{0.98}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.98}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.72}\textcolor[HTML]{008000}{$\uparrow$} 
% & 0.71\textcolor[HTML]{FF0000}{$\downarrow$} 
% & \textbf{0.67}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.67}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.61}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.62}\textcolor[HTML]{008000}{$\uparrow$} \\
% \hline

% \multirow{2}{*}{Qwen3-VL-4B}
% & PET + CT
% & 0.60 & 0.79 & 0.31 & 0.34 & 0.29 & 0.20 & \textbf{0.67} & \textbf{0.64} \\
% & PET/CT
% & \textbf{0.92}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.89}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.68}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.68}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.66}\textcolor[HTML]{008000}{$\uparrow$} 
% & \textbf{0.63}\textcolor[HTML]{008000}{$\uparrow$} 
% & 0.63\textcolor[HTML]{FF0000}{$\downarrow$} 
% & 0.62\textcolor[HTML]{FF0000}{$\downarrow$} \\
% \hline
% \end{tabular}
% \end{adjustbox}

% \caption{Comparison of performance (F1-score) between \textbf{PET+CT} (input PET \& CT images separately) and fused PET/CT inputs across steps in both English \& Vietnamese.}
% \label{tab:pet_ct_vs_petct}
% \end{table}




As shown in Table~\ref{tab:pet_ct_vs_petct}, clinically fused PET/CT inputs consistently outperform simple PET+CT concatenation across models. For Gemini~2.5~Flash, PET/CT fusion yields a large gain at Step~1 (VI), improving F1 from 0.79 to 0.98, and also improves fine-grained reasoning at Step~3 (EN) from 0.62 to 0.67. Similarly, Qwen3-VL-4B benefits substantially from PET/CT fusion, with Step~3 (EN) F1 increasing from 0.20 to 0.63, more than a threefold improvement. These results indicate that clinically grounded PET/CT fusion significantly enhances cross-modal alignment and fine-grained reasoning compared to naïve modality concatenation.


\begin{table}[h]
\centering
\large
\setlength{\tabcolsep}{5.2pt}
\renewcommand{\arraystretch}{1.2}

\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{l !{\vrule width 0.8pt} c !{\vrule width 0.8pt}
cc !{\vrule width 0.8pt}
cc !{\vrule width 0.8pt}
cc !{\vrule width 0.8pt}
cc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Input}} &
\multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 1}} &
\multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 2}} &
\multicolumn{2}{c!{\vrule width 0.8pt}}{\textbf{Step 3}} &
\multicolumn{2}{c}{\textbf{Step 4}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
%\hline
& & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} & \textbf{VI} & \textbf{EN} \\
\hline

\multirow{2}{*}{\makecell[l]{Med\\Flamingo}}
& PET + CT
& -- & 0.64 & -- & 0.64 & -- & \textbf{0.66} & -- & \textbf{0.66} \\
& PET/CT
& -- & \textbf{0.77}\textcolor[HTML]{008000}{$\uparrow$} 
& -- & \textbf{0.66}\textcolor[HTML]{008000}{$\uparrow$} 
& -- & 0.63\textcolor[HTML]{FF0000}{$\downarrow$} 
& -- & 0.59\textcolor[HTML]{FF0000}{$\downarrow$} \\
\hline

\multirow{2}{*}{\makecell[l]{Gemini 2.5\\Flash}}
& PET + CT
& 0.79 & 0.81 & 0.68 & \textbf{0.72} & 0.62 & 0.62 & 0.51 & 0.52 \\
& PET/CT
& \textbf{0.98}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.98}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.72}\textcolor[HTML]{008000}{$\uparrow$} 
& 0.71\textcolor[HTML]{FF0000}{$\downarrow$} 
& \textbf{0.67}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.67}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.61}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.62}\textcolor[HTML]{008000}{$\uparrow$} \\
\hline

\multirow{2}{*}{\makecell[l]{Qwen3\\VL-4B}}
& PET + CT
& 0.60 & 0.79 & 0.31 & 0.34 & 0.29 & 0.20 & \textbf{0.67} & \textbf{0.64} \\
& PET/CT
& \textbf{0.92}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.89}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.68}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.65}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.66}\textcolor[HTML]{008000}{$\uparrow$} 
& \textbf{0.62}\textcolor[HTML]{008000}{$\uparrow$} 
& 0.63\textcolor[HTML]{FF0000}{$\downarrow$} 
& 0.62\textcolor[HTML]{FF0000}{$\downarrow$} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of performance (F1-score) between PET+CT (separate inputs) and fused PET/CT across steps in both English and Vietnamese.}
\label{tab:pet_ct_vs_petct}
\end{table}






% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/EN_VI_v3.png}
%     \caption{Performance of models between Vietnamese \& English dataset}
%     \label{fig:placeholder}
% \end{figure}
% Table~\ref{tab:internal_vs_external} shows that injecting prior or external knowledge mainly increases recall, often at the cost of precision, indicating a shift from evidence verification toward acceptance.

% For Qwen3-VL-4B, prior knowledge boosts Step~2 recall (0.82$\rightarrow$0.94) while preserving F1 (0.68), but external knowledge degrades Step~4 performance (F1 drops to 0.52). Combining both sources stabilizes Step~3 (F1=0.67) but does not recover late-stage accuracy. Med-Flamingo exhibits strong early recall gains (Step~2 recall up to 0.96) but consistent degradation at Steps~3--4 (F1 decreases from 0.63 to 0.59--0.62), suggesting over-reliance on auxiliary knowledge during fine-grained reasoning. 

% Gemini~2.5~Flash is comparatively robust: external knowledge improves Step~4 F1 (0.61$\rightarrow$0.65), whereas prior knowledge alone degrades mid-stage performance (Step~3 F1 drops to 0.54). Overall, knowledge augmentation acts as a double-edged signal, improving coverage but weakening late-stage grounding, particularly for medical-specialized models.
% This table shows that a clinically aligned PET/CT fused overlay is generally more effective than providing PET and CT as separate inputs (PET+CT), especially for general-purpose VLMs.

% For Gemini 2.5 Flash, PET/CT fusion yields consistent gains across multiple stages: clear improvements in Steps 1–3 (in both VI and EN), with a small gain in Step 4, indicating that fusion helps the model jointly integrate metabolic (PET) and anatomical (CT) cues for consistency verification.

% For Qwen3-VL-4B, PET/CT fusion produces large improvements in Steps 1–3 (particularly Step 1), while Step 4 slightly decreases, suggesting fusion primarily benefits stages requiring visual grounding (anatomy/lesion/feature), whereas synthesis remains challenging.

% For Med-Flamingo, PET/CT fusion improves Steps 1–2 (EN increases) but drops in Steps 3–4, implying that fusion is not universally better for medical-specialized models; however, the main takeaway remains that the clearest benefit appears for non-specialized models.

% Overall, the clinical overlay fusion is not just a presentation choice but a meaningful input design that better aligns with routine PET/CT reading, enabling models to exploit PET uptake together with CT anatomy more effectively than two disconnected images.



%  When a rationale is added, models no longer rely purely on visual evidence; the extra text steers the decision, making consistency judgments less tightly grounded in the image.

% Clinician-written rationales are often more harmful because they sound clinically standard, coherent, and report-like, which makes models more likely to trust them and “legitimize” an incorrect statement.

%  The main failure signal is a drop in recall: models miss more hallucinations, i.e., they are more likely to accept an incorrect statement as consistent with the image when a clinician rationale is present.

%  Compared to the no-explanation setting, LLM-generated rationales do not show a consistent degradation trend because they are often less clinically constrained and sometimes not persuasive enough to flip the model’s judgment. They can be generic, exhibit machine-like patterns, lack realistic clinical constraints, or even provide cues that still push the model toward an “inconsistent” decision. As a result, recall is typically not pulled down as strongly as with clinician rationales.

%  Med-Flamingo is an exception: it is more sensitive to LLM-generated rationales (with a sharp performance drop), suggesting that vulnerability is not determined only by “persuasiveness,” but also by textual distribution shift and how a model fuses visual and textual signals.

%  Overall, models can be persuaded by a plausible narrative rather than verifying evidence, and clinician rationales act as a stronger adversary than LLM rationales. Behaviorally, clinician rationales function as a high-quality adversarial intermediate explanation: they do not need to match the image, only to be clinically plausible enough to pass the model’s language prior, revealing a “persuasion over evidence” failure mode.
% \begin{table}[H]
% \centering
% \caption{Add explanation vs. no explanation}
% \label{tab:add_expl_no_expl_cols}
% \scriptsize
% \setlength{\tabcolsep}{2.5pt} % giảm spacing
% \renewcommand{\arraystretch}{1.1}

% \begin{adjustbox}{width=\columnwidth}
% \begin{tabular}{l !{\vrule width 0.6pt}
% ccc !{\vrule width 0.6pt}
% ccc !{\vrule width 0.6pt}
% ccc !{\vrule width 0.6pt}
% ccc !{\vrule width 0.6pt}
% ccc}
% \toprule
% \textbf{Setting} &
% \multicolumn{3}{c!{\vrule width 0.6pt}}{\textbf{Med-Flamingo}} &
% \multicolumn{3}{c!{\vrule width 0.6pt}}{\textbf{Gemini 2.5 Pro}} &
% \multicolumn{3}{c!{\vrule width 0.6pt}}{\textbf{Gemini 2.5 Flash}} &
% \multicolumn{3}{c!{\vrule width 0.6pt}}{\textbf{MedM-VL 3D}} &
% \multicolumn{3}{c}{\textbf{MedM-VL 2D}} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
% & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline
% No explanation
% & 0.49 & 0.84 & 0.62
% & 0.50 & 0.88 & 0.64
% & 0.50 & 0.96 & 0.66
% & 0.48 & 0.90 & 0.63
% & 0.38 & 0.60 & 0.46 \\
% LLM explanation
% & 0.20 & 0.24 & 0.22
% & 0.51 & 0.96 & 0.67
% & 0.53 & 0.98 & 0.69
% & 0.47 & 0.86 & 0.60
% & 0.36 & 0.57 & 0.45 \\
% Clinical rationale
% & 0.43 & 0.76 & 0.55
% & 0.48 & 0.70 & 0.57
% & 0.47 & 0.74 & 0.57
% & 0.42 & 0.72 & 0.53
% & 0.37 & 0.58 & 0.45 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}


==> Document/7.tex <==


% \subsection{Step-wise Hallucination Evaluation}
% \label{sec:stepwise_formulation}

% We formalize hallucination detection in medical vision--language models (VLMs) as a step-wise visual--textual consistency evaluation problem. Given a PET/CT study, the evaluation algorithm decomposes clinical interpretation into four sequential diagnostic stages:
% anatomical mapping ($s=1$), lesion identification ($s=2$), feature characterization ($s=3$), and diagnostic synthesis ($s=4$).
% Each stage is evaluated independently to isolate hallucination behaviors specific to different levels of clinical reasoning.

% \paragraph{Step-wise data construction.}
% For a given stage $s$, we construct a dataset
% \[
% \mathcal{D}_s=\left\{(I_s^{(i)},\, t_s^{(i)},\, y_s^{(i)})\right\}_{i=1}^{N_s},
% \]
% where $I_s$ denotes the stage-specific visual input (multi-view 2D images, 3D volumetric input, or fused PET/CT),
% $t_s$ is a textual statement to be verified against the image evidence,
% and $y_s\in\{0,1\}$ is the consistency label, with $y_s=1$ indicating a hallucination (i.e., the statement is inconsistent with the visual input).

% \paragraph{Clinically grounded hallucinated statement generation.}
% To systematically probe hallucination behaviors, we generate hallucinated statements through clinically grounded corruption operators.
% Let $t_s^{\star}$ denote a factual, image-consistent statement at stage $s$.
% A hallucinated counterpart $\tilde{t}_s$ is generated by applying a stage-specific transformation
% \begin{equation}
% \tilde{t}_s = \mathcal{T}_s(t_s^{\star}; \xi_s),
% \label{eq:corruption}
% \end{equation}
% where $\mathcal{T}_s$ introduces clinically plausible but image-incompatible modifications, and $\xi_s$ denotes random or controlled perturbation parameters.
% Specifically, $\mathcal{T}_1$ produces anatomical mismatches, $\mathcal{T}_2$ generates false or missing abnormalities,
% $\mathcal{T}_3$ fabricates quantitative lesion attributes (e.g., SUV$_{\max}$, lesion size),
% and $\mathcal{T}_4$ synthesizes unsupported disease claims.
% Each sample is labeled as $y_s=0$ if $t_s=t_s^{\star}$ and $y_s=1$ if $t_s=\tilde{t}_s$.

% \paragraph{Consistency judgment.}
% At inference time, a vision--language model $f_{\theta}$ is queried to judge the consistency between the visual input and the textual statement.
% The model predicts the probability that a statement is hallucinatory as
% \begin{equation}
% p_{\theta}(y=1 \mid I_s,\, t_s,\, k_s),
% \label{eq:consistency}
% \end{equation}
% where $k_s$ denotes an optional knowledge context.
% The predicted label $\hat{y}_s$ is obtained via thresholding or deterministic parsing of the model output:
% \begin{equation}
% \hat{y}_s = \mathbb{I}\!\left[p_{\theta}(y=1 \mid I_s, t_s, k_s) \ge \tau \right],
% \label{eq:decision}
% \end{equation}
% with $\tau$ being a fixed decision threshold.

% \paragraph{Controlled knowledge injection.}
% For stages $s \ge 2$, the algorithm supports controlled knowledge injection to analyze the role of intermediate information in hallucination detection.
% The knowledge context is defined as
% \begin{equation}
% k_s = \left[k_s^{\text{prior}};\, k_s^{\text{ext}}\right],
% \label{eq:knowledge}
% \end{equation}
% where $k_s^{\text{prior}}$ is derived from deterministic ground-truth outputs of earlier stages,
% and $k_s^{\text{ext}}$ corresponds to curated or retrieved external medical knowledge introduced only when clinically meaningful.
% This formulation enables systematic comparison between no-knowledge, prior-only, external-only, and combined knowledge settings.

% \paragraph{Rationale vulnerability and persuasion over evidence.}
% To assess susceptibility to persuasive language, the algorithm augments the input statement with an intermediate rationale $r_s$,
% yielding a rationale-augmented query $[t_s; r_s]$.
% The corresponding hallucination probability becomes
% \begin{equation}
% p_{\theta}(y=1 \mid I_s,\,[t_s; r_s],\, k_s).
% \label{eq:rationale_pred}
% \end{equation}
% We model rationale injection as a constrained linguistic perturbation, where $r_s$ is required to satisfy a clinical plausibility constraint
% $\mathcal{C}(r_s) \ge \gamma$, ensuring that the rationale remains fluent and clinically realistic.

% Hallucination vulnerability is quantified via the recall on hallucinated samples:
% \begin{equation}
% R_s = \Pr(\hat{y}_s = 1 \mid y_s = 1),
% \label{eq:recall}
% \end{equation}
% and the recall drop induced by rationale injection is defined as
% \begin{equation}
% \Delta R_s(r) = R_s(\varnothing) - R_s(r),
% \label{eq:recall_drop}
% \end{equation}
% which directly measures the increase in missed hallucinations caused by persuasive intermediate explanations.
% A positive $\Delta R_s(r)$ indicates that the model is being persuaded by linguistic rationales despite contradictory visual evidence,
% revealing a persuasion-over-evidence failure mode.



% \paragraph{Evaluation metrics.}
% Across all stages, hallucination detection performance is summarized using Precision, Recall, and F1-score,
% computed with hallucination ($y=1$) as the positive class.
% By aggregating results across stages and experimental conditions, the proposed formulation enables fine-grained analysis of
% hallucination propagation, step-specific failure modes, and robustness factors in medical VLMs.





% VER2 
% \begin{algorithm}[t]
% \caption{Med-StepBench: Step-wise Hallucination Evaluation with Knowledge and Rationale Attacks}
% \label{alg:medstepbench_full}
% \footnotesize
% \setlength{\baselineskip}{0.5\baselineskip} 
% \begin{algorithmic}[1]
% \REQUIRE
% Step-wise benchmark splits $\{\mathcal{S}_s\}_{s=1}^{4}$ over 3D oncologic PET/CT studies, each study providing
% multi-view 2D slices $\mathbf{X}$ and a registered 3D volume $\mathbf{V}$;
% clinician-verified factual evidence $\mathrm{Ev}(u,s)$ (reports/annotations);
% stage-specific corruption operators $\{\mathcal{T}_s\}_{s=1}^{4}$;
% knowledge builders $\phi_s(\cdot)$ (prior) and $\psi_s(\cdot)$ (external/RAG);
% rationale sources: $\mathcal{G}^{\text{llm}}_s$ and clinician rationales $\mathcal{G}^{\text{clin}}_s$;
% VLM under test $f_\theta$; prompt constructor $\mathrm{Prompt}(\cdot)$; output parser $\mathrm{Parse}(\cdot)$.
% \ENSURE
% Per-step metrics $\mathrm{Precision}_{s,\omega}$, $\mathrm{Recall}_{s,\omega}$, $\mathrm{F1}_{s,\omega}$ for all settings $\omega$;
% rationale vulnerability scores $\Delta \mathrm{Recall}_{s}(\cdot)$.

% \vspace{2pt}
% \STATE Define evaluation setting space $\Omega$ as combinations of:
% \STATE \hspace{6pt} \textbf{(A) Visual mode:} \texttt{2D}, \texttt{3D}, \texttt{2D+3D};
% \textbf{(B) PET/CT input:} \texttt{PET+CT} vs. \texttt{PET/CT fused};
% \textbf{(C) Knowledge:} \texttt{None}, \texttt{+Prior}, \texttt{+Ext}, \texttt{+Both};
% \textbf{(D) Rationale:} \texttt{No}, \texttt{LLM}, \texttt{Clinician}.

% \FOR{$s \leftarrow 1$ \TO $4$} \COMMENT{Step-wise evaluation: anatomical $\rightarrow$ lesion $\rightarrow$ attributes $\rightarrow$ diagnosis}
%     \FOR{each setting $\omega \in \Omega$}
%         \STATE Initialize confusion counts: $\mathrm{TP}\leftarrow 0$, $\mathrm{FP}\leftarrow 0$, $\mathrm{FN}\leftarrow 0$.
%         \FOR{each study/sample $u \in \mathcal{S}_s$}

%             \STATE \textbf{(1) Visual input selection (2D/3D and PET/CT fusion).}
%             \STATE $I_s \leftarrow \mathrm{BuildVisual}(u, s, \omega)$
%             \COMMENT{e.g., $I_s=\mathbf{X}$ (2D), $I_s=\mathbf{V}$ (3D),
%             or $\Phi(\mathrm{PET},\mathrm{CT})$ (fused overlay) vs. $(\mathrm{PET},\mathrm{CT})$}

%             \STATE \textbf{(2) Construct factual statement from clinician-verified evidence.}
%             \STATE $t^{\star}_s \leftarrow \mathrm{BuildFactualStatement}(\mathrm{Ev}(u,s))$

%             \STATE \textbf{(3) Generate hallucinated counterpart via step-specific corruption.}
%             \STATE Sample label $y_s \sim \mathrm{Bernoulli}(\pi_s)$ \COMMENT{$y_s=1$: hallucination/inconsistent}
%             \IF{$y_s = 0$}
%                 \STATE $t_s \leftarrow t^{\star}_s$
%             \ELSE
%                 \STATE $t_s \leftarrow \mathcal{T}_s(t^{\star}_s;\mathrm{Ev}(u,s))$
%                 \COMMENT{$\mathcal{T}_1$: anatomical mismatch; $\mathcal{T}_2$: false/missing abnormality;
%                 $\mathcal{T}_3$: fabricated attributes; $\mathcal{T}_4$: false disease claim}
%             \ENDIF

%             \STATE \textbf{(4) Controlled knowledge injection (RQ2).}
%             \STATE $k_s \leftarrow \varnothing$
%             \IF{$s \ge 2$}
%                 \STATE $k^{\text{prior}}_s \leftarrow \varnothing$; $k^{\text{ext}}_s \leftarrow \varnothing$
%                 \IF{$\omega$ includes prior knowledge}
%                     \STATE $k^{\text{prior}}_s \leftarrow \phi_s(o^{\star}_{<s}(u))$
%                     \COMMENT{deterministic ground-truth outputs from earlier steps}
%                 \ENDIF
%                 \IF{$\omega$ includes external knowledge}
%                     \STATE $k^{\text{ext}}_s \leftarrow \psi_s(\mathcal{E}_s, u)$
%                     \COMMENT{curated evidence / RAG; stage-dependent}
%                 \ENDIF
%                 \STATE $k_s \leftarrow \mathrm{Concat}(k^{\text{prior}}_s, k^{\text{ext}}_s)$
%             \ENDIF

%             \STATE \textbf{(5) Rationale attack injection (RQ3).}
%             \STATE $r_s \leftarrow \varnothing$
%             \IF{$\omega$ includes LLM rationale}
%                 \STATE $r_s \leftarrow \mathcal{G}^{\text{llm}}_s(u, I_s, t_s)$
%             \ELSIF{$\omega$ includes clinician rationale}
%                 \STATE $r_s \leftarrow \mathcal{G}^{\text{clin}}_s(u, s)$
%             \ENDIF

%             \STATE \textbf{(6) Query VLM for consistency judgment.}
%             \STATE $\textsc{prompt} \leftarrow \mathrm{Prompt}(s, t_s, k_s, r_s)$
%             \STATE $z \leftarrow f_\theta(I_s,\ \textsc{prompt})$
%             \STATE $\hat{y}_s \leftarrow \mathrm{Parse}(z)$
%             \COMMENT{$\hat{y}_s=1$ means predicted hallucination/inconsistent}

%             \STATE \textbf{(7) Update confusion counts (positive = hallucination).}
%             \IF{$\hat{y}_s=1 \land y_s=1$} \STATE $\mathrm{TP}\leftarrow \mathrm{TP}+1$
%             \ELSIF{$\hat{y}_s=1 \land y_s=0$} \STATE $\mathrm{FP}\leftarrow \mathrm{FP}+1$
%             \ELSIF{$\hat{y}_s=0 \land y_s=1$} \STATE $\mathrm{FN}\leftarrow \mathrm{FN}+1$
%             \ENDIF
%         \ENDFOR

%         \STATE \textbf{(8) Compute step-wise hallucination metrics.}
%         \STATE $\mathrm{Precision}_{s,\omega} \leftarrow \frac{\mathrm{TP}}{\mathrm{TP}+\mathrm{FP}+\epsilon}$
%         \STATE $\mathrm{Recall}_{s,\omega} \leftarrow \frac{\mathrm{TP}}{\mathrm{TP}+\mathrm{FN}+\epsilon}$
%         \STATE $\mathrm{F1}_{s,\omega} \leftarrow \frac{2\,\mathrm{Precision}_{s,\omega}\,\mathrm{Recall}_{s,\omega}}{\mathrm{Precision}_{s,\omega}+\mathrm{Recall}_{s,\omega}+\epsilon}$

%     \ENDFOR

%     \STATE \textbf{(9) Rationale vulnerability summary at step $s$ (persuasion-over-evidence).}
%     \STATE Let $\omega_{\text{no}}$ be the setting identical to $\omega$ but with \texttt{No rationale}.
%     \STATE Let $\omega_{\text{r}}$ be the setting identical to $\omega$ but with rationale source $\texttt{r}\in\{\texttt{LLM},\texttt{Clinician}\}$.
%     \STATE $\Delta \mathrm{Recall}_{s}(\texttt{r}) \leftarrow \mathrm{Recall}_{s,\omega_{\text{no}}} - \mathrm{Recall}_{s,\omega_{\text{r}}}$
% \ENDFOR

% \RETURN $\{\mathrm{Precision}_{s,\omega}, \mathrm{Recall}_{s,\omega}, \mathrm{F1}_{s,\omega}\}$ and $\{\Delta \mathrm{Recall}_{s}(\texttt{r})\}$.
% \end{algorithmic}
% \end{algorithm}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/Models_steps_comparision2.png}
%     \caption{Performance of models during steps (F1-score).}
% %    \Amir{It is better you give me the table information with 2 floating points, so on top of the bar, I update the percentage with 2 floating points}
% \reza{the values font is too small, same for legend}
%     \label{fig:step_wise}
% \end{figure}






% Requires:
% \usepackage{booktabs}      % for \cmidrule
% \usepackage{multirow}
% \usepackage{adjustbox}
% \usepackage[table]{xcolor} % for \rowcolor, \cellcolor

% Requires:
% \usepackage{booktabs}      % for \cmidrule
% \usepackage{multirow}
% \usepackage{adjustbox}
% \usepackage[table]{xcolor} % for \textcolor

Despite its contributions, this study has several limitations. First, Med-StepBench focuses on oncologic PET/CT and it may not directly generalize to other imaging modalities such as MRI, ultrasound, or non-oncologic applications. Although the step-wise evaluation framework is a general methodology, extending the benchmark to additional modalities and disease contexts remains an important direction for future work. Second, while our step-level labels enable a new assessment of grounding at each diagnostic stage, we do not yet model hallucination propagation along a model’s true internal reasoning, which may differ from the prescribed clinical workflow.
% Third, Med-StepBench is formulated as step-wise consistency judgment rather than end-to-end report generation, and thus does not provide full verification of free-form clinical reports.
We view Med-StepBench as a first step toward systematic, step-aware evaluation of hallucination in medical vision–language models, and anticipate that future extensions will address these limitations.

